Focal Surface Holographic Light Transport using Learned Spatially Adaptive Convolutions

Computer-Generated Holography (CGH) is a set of algorithmic methods for identifying holograms that reconstruct Three-Dimensional (3D) scenes in holographic displays. CGH algorithms decompose 3D scenes into multiplanes at different depth levels and rely on simulations of light that propagated from a source plane to a targeted plane. Thus, for n planes, CGH typically optimizes holograms using n plane-to-plane light transport simulations, leading to major time and computational demands. Our work replaces multiple planes with a focal surface and introduces a learned light transport model that could propagate a light field from a source plane to the focal surface in a single inference. Our learned light transport model leverages spatially adaptive convolution to achieve depth-varying propagation demanded by targeted focal surfaces. The proposed model reduces the hologram optimization process up to 1.5x, which contributes to hologram dataset generation and the training of future learned CGH models.

==> latex/sec2-relatedworks.tex <==
\section{Related Work}



% \subsection{Conventional Light Propagation }

% Conventional light propagation models in~\CGH~are based on Rayleigh-Sommerfeld diffraction~\cite{RayleighSommerfeld}, a method established for accurate light field evaluations in both far-field and near-field. The numerical solution to the Rayleigh–Sommerfeld integral is achievable via methods like angular spectrum~\cite{bandLimited} or direct integration~\cite{DirectRayleighSommerfeld}. Based on the two methods, various light propagation models are designed. These models can be classified according to the type of target surface they address, which includes propagation between parallel planes~\cite{bandLimited,shiftedFresnel,randomVectors} and the propagation between non-parallel planes~\cite{rotationalplane,tiltedPlane,tiltedplaneAS}. Particularly, the arbitrarily tilted plane propagation method~\cite{tiltedplaneAS} facilitates the simulation of three-dimensional surface objects~\cite{trianglemeshmodeled}. However, these methods are typically confined to simulating wave propagation onto 2D planes, leading to a two-stage process for simulating arbitrary surface propagation. The first stage involves using simulation functions to project holograms onto various target planes. The second stage consists of aggregating all focus contributions from each target plane. Meanwhile, Lohmann lens-based diffraction model~\cite{chang2024split} has been proposed, but such methods require long optical paths, which makes it harder to miniaturize. In our work, we take a step further by developing a learned focal surface light transport model. This model directly propagates complex fields from the hologram plane to both flat 2D planes and 3D depth-varying focal surfaces.



\subsection{Learned Light Propagation}
In learning-based~\CGH, diverse light propagation models have been developed for hologram optimization. These models are broadly categorized into plane-to-plane and plane-to-multiplane simulations. For the former, a signal-learned kernel in the frequency domain~\cite{learnedLightTransport} was introduced to replace the angular spectrum kernel, enhancing light propagation simulation in real-world experimental settings. Additionally, to accurately represent optical aberrations in light paths, a convolution-based network~\cite{neuralHolography} was designed for practical light transport simulation. Similar work can be found in~\cite{chakravarthula2020learned} which learned the deviations of the real display from the ideal light transport for simulation. In plane-to-multiplane simulations, inspired by previous works~\cite{neuralHolography,chakravarthula2020learned}, neural 3D holography~\cite{neural3dHolography} introduced a plane-to-multiplane transport model that utilizes the angular spectrum~\cite{bandLimited} method for light propagation across multiple planes. Subsequently, a U-Net-based network is applied to each target plane image for refinement. Meanwhile, MDHGN~\cite{lee2020deep} simulated plane-to-multiplane light transport based on a residual network architecture~\cite{residualNetwork}, and the datasets for training were generated by the angular spectrum method~\cite{bandLimited}. While current plane-to-multiplane light propagation simulations facilitate 3D spatial light propagation, they are still based on plane-to-plane interaction.


% \subsection{Content-Adaptive Convolution}
% Convolution is the basic operation in~\CNN and is characterized by spatial sharing and content agnostic~\cite{pixeladaptive}. To address these two drawbacks, serious content adaptive convolution has been proposed. \DFN~\cite{dynamicFilter,kernelpredicting} using a separate sub-network to predict convolutional filter weights at each pixel, achieving position-specific and content-adaptive convolution. However, it is difficult to predict a serious kernel for an entire network. To solve this problem both pixel-adaptive convolution and windowing decomposition convolution have been proposed.  Windowing decomposition convolution~\cite{zheng2021windowing} decomposes the content of the convolution window, using different decomposition values to achieve content-adaptive convolution. But still based on spatial invariant kernel. Pixel-adaptive convolution~\cite{pixeladaptive} multiplies standard convolution kernels with  Gaussian kernels to achieve spatially adaptive operation. However, the spatially adaptive kernel is shared across all channels and is limited by the specific selected Gaussian kernel function.








